Wisdom of the Crowd or Wisdom of a Few? An Analysis of Users' Content Generation

In this paper we analyze how user generated content (UGC) is created, challenging the well known {\it wisdom of crowds} concept. Although it is known that user activity in most settings follow a power law, that is, few people do a lot, while most do nothing, there are few studies that characterize well this activity. In our analysis of datasets from two different social networks, Facebook and Twitter, we find that a small percentage of active users and much less of all users represent 50\% of the UGC. We also analyze the dynamic behavior of the generation of this content to find that the set of most active users is quite stable in time. Moreover, we study the social graph, finding that those active users are highly connected among them. This implies that most of the wisdom comes from a few users, challenging the independence assumption needed to have a wisdom of crowds. We also address the content that is never seen by any people, which we call digital desert, that challenges the assumption that the content of every person should be taken in account in a collective decision. We also compare our results with Wikipedia data and we address the quality of UGC content using an Amazon dataset. At the end our results are not surprising, as the Web is a reflection of our own society, where economical or political power also is in the hands of minorities.

==> 06_discussion.tex <==

%\begin{figure}[t!]
%\centering
%\hspace*{-.5cm}
%\epsfig{file=images/ranking_vs_articles.png, width=.97\linewidth}
%\epsfig{file=images/webtraffic_people_per_month.jpg, width=\columnwidth}
%\caption{Distribution of articles with respect to top Wikipedia editors.}
%\caption{Distribution of articles with respect to top Wikipedia editors (left) and distribution of unique users per month in the most visited sites of the USA (right).}
%\label{fig:wiki}
%\end{figure}


\section{Discussion and Future Work}

We can partially compare our results in social networks to the content generation process of Wikipedia. Indeed, according to data published by Wikipedia itself, the top 10,000 editors produce the 33\% of content editions. Considering that there are almost 20.8 million registered editors, the top editors represent just 0.04\% of them. 
% As it is estimated than 29\% of the valid Wikipedia edits are done by non-registered editors,\footnote{\url{http://en.wikipedia.org/wiki/File:Top_editors_(including_bots)_compared_to_the_rest_of_the_community,_8_January_2014.svg}} we can estimate that the number of active editors is about \notas{YY} millions. That is, in the case of Wikipedia the bias in the user activity is even higher. 
As the number of passive users, that is, people that use Wikipedia but do not contribute with content, is more than one billion, the percentage of active editors with respect to the total number of users is negligible. Something similar happens with the creation of the almost 4.5 million Wikipedia articles in English, the 2,005 most prolific authors account to the creation of 50\% of the articles\cite{fewwikipedia}. This is less than 0.01\% of registered editors, and this number would be even smaller if the non-registered users could be taken into account. 

%Figure~\ref{fig:wiki} shows the distribution which can be modeled by a power law of exponent -0.89.


%We can also estimate a lower bound for the content that is never seen in for the case of the Twitter dataset. In fact, a lower bound for the digital desert can be computed as the percentage of content generated by people that has no followers. This percentage of people is only 0.06\% for the {\it wise} group but 20.58\% for the {\it others} group. This accounts for 0.03\% and 1.08\% of the whole content, respectively. Hence, the digital dessert in our dataset is at least 1.11\%. Although small, this implies that the opinion of some people is not really considered and hence is not part of the collective wisdom. Hence, we have a partial wisdom of crowds.

%We can compare this number by extrapolating the distribution of website traffic in the USA according to Quantcast\footnote{https://www.quantcast.com/top-sites/} given in Figure~\ref{fig:wiki}(right). This distribution follows a power law of exponent -0.94. This implies that around the website at rank \notas{Y} the unique numbers of visitors per month is less than 1.  If we estimate the USA websites in 20 millions, that means that \notas{Z\%} of them have basically no traffic. That is, a much bigger digital desert.
%Based on our results we can represent all these ideas in a metaphorical map of the wisdom behind the users as shown in Figure~\ref{fig:map}, where the vertical axis represent all users in a logarithmic scale while the horizontal axis represent the generation of content for each user (that is, with a 90 degree rotation to the right we have a normal graph that reverses the order of users of Figure~\ref{fig:acivity-vs-active}).

